Scalable Learning-Based Sampling Optimization for Compressive Dynamic MRI

Compressed sensing applied to magnetic resonance imaging (MRI) allows to reduce the scanning time by enabling images to be reconstructed from highly undersampled data. In this paper, we tackle the problem of designing a sampling mask for an arbitrary reconstruction method and a limited acquisition budget. Namely, we look for an optimal probability distribution from which a mask with a fixed cardinality is drawn. We demonstrate that this problem admits a compactly supported solution, which leads to a deterministic optimal sampling mask. We then propose a stochastic greedy algorithm that (i) provides an approximate solution to this problem, and (ii) resolves the scaling issues of [1,2]. We validate its performance on in vivo dynamic MRI with retrospective undersampling, showing that our method preserves the performance of [1,2] while reducing the computational burden by a factor close to 200.

==> ICASSP_Scalable_MRI_arXiv copy/01-introduction.tex <==
%!TEX root = ms.tex
\vspace{-4mm}
\section{Introduction}
\vspace{-.3cm}
%{\bf INTRODUCTION, SETUP AND LITERATURE REVIEW SHOULD BE IN ONE PAGE} 
Dynamic Magnetic Resonance Imaging (dMRI) is a powerful tool in medical imaging, which allows for non-invasive monitoring of tissues over time. A main challenge to the quality of dMRI examinations is the inefficiency of data acquisition that limits temporal and spatial resolutions. In the presence of moving tissues, such as in cardiac MRI, the trade-off between spatial and temporal resolution is further complicated by the need to perform breath-holds to minimize motion artifacts \cite{saeed2015cardiac}.


In the last decade, the rise of Compressed Sensing (CS) has significantly contributed to overcoming these problems.  CS allows for a successful reconstruction from undersampled measurements, provided that they are incoherent \cite{candes2006stable,donoho2006compressed} and that the data can be sparsely represented in some domain. In dMRI, samples are acquired in the $k$-$t$ space (spatial frequency and time domain), and can be sparsely represented in the $x$-$f$ domain (image and temporal Fourier transform domain). %the temporally neighboring images are highly correlated, which enables the signal to be sparsely represented in the x-f domain (image and temporal Fourier transform domain). 
Many algorithms have exploited this framework with great success (see \cite{lustig2006kt,jung2009k,otazo2010combination,lingala2011accelerated, feng2014golden, caballero2014dictionary, otazo2015low, jin2016general, schlemper2018deep} and the references therein). %Some works also exploit dictionary learning, where they design a compact sparsifying transform \cite{lingala2013blind, wang2014compressed, caballero2014dictionary}, and some focus on low-rank approaches \cite{lingala2011accelerated, yoon2014motion, otazo2015low, jin2016general}.


While CS theory mostly focuses on fully random measurements \cite{candes2006robust}, the practical implementations have generally exploited \textit{random variable-density sampling}, based on drawing random samples from a parametric distribution (typically polynomial or Gaussian) which reasonably imitates the energy distribution in the $k$-$t$ space \cite{lustig2007sparse, jung2007improved}. %  This was proposed by Lustig et al. for static MRI \cite{lustig2007sparse}, and applied to dMRI by Jung et al. \cite{jung2007improved}, 
%Common practices have included adding a slight offset prevent the distribution from having extremely small probabilities at high-frequencies, as well as acquired a few low-frequency \mbox{k-space} samples at the Nyquist rate.
 While all these approaches allow to quickly design masks which yield a great improvement over fully random sampling, prescribed by the theory of CS, they \di remain largely heuristic; \ii ignore the anatomy of interest; \iii ignore the reconstruction algorithm; \iv require careful tuning of their various parameters, and \dv do not necessarily use a fixed number of readouts per frame.
%and the distributions considered have typically been either polynomial \cite{lustig2007sparse, kim2012accelerated, tremoulheac2014dynamic, weizman2015compressed} or Gaussian \cite{jung2009k, otazo2010combination, caballero2014dictionary,otazo2015low,jin2016general,schlemper2018deep}. Common practices have included adding a slight offset prevent the distribution from having extremely small probabilities at high-frequencies, as well as acquired a few low-frequency \mbox{k-space} samples at the Nyquist rate. While all these approaches allow to quickly design masks which yield a great improvement over fully random sampling, prescribed by the theory of CS, they remain fully heuristic and ignore the anatomy and the reconstruction algorithm at hand. They also require careful tuning of their various parameters, and do not necessarily satisfy the additional design constrain of using a fixed number of readouts per frame in dMRI.

%The variable-density based methods commonly used in dMRI perform well, but have several weaknesses, already highlighted in \cite{gozcu2017, gozcu2019rethinking} for static MRI. They require parameters to be tuned, such as decay rate of the polynomial, the standard deviation of the Gaussian distribution or the number of central phase encodes and arbitrarily constrain the sampling patterns to a model without any theoretical justification. Moreover, it is unclear which sampling density will be most effective for a given anatomy and reconstruction rule. Also, the idea of randomizing the acquisition is in itself questionable, as in practice, one would desire to design a fixed sampling pattern that we will know to perform well for a specific anatomy across many subjects. Finally, some variable-density methods, such as Poisson Disc Sampling \cite{vasanawala2011practical}, do not use a fixed number of readouts per frame, which complicates their hardware implementation for dynamic MRI \cite{ahmad2015variable}. Indeed, undersampling some frames more heavily than others might result in missing critical temporal information.


%. A few works later specifically attempted at designing sampling patterns for dMRI \cite{ahmad2015variable, li2018dynamic}.


In the present work, we show that the problem of finding an optimal mask sampling distribution which contains $n$ out of $p$ possible locations admits a solution compactly supported on $n$ elements. This demonstrates that our previously proposed framework in \cite{gozcu2017, gozcu2019rethinking}, which searches for an approximately optimal sampling mask, is in fact looking for a solution to the more general problem of finding an optimal measurement distribution.
In addition, we propose a \textit{scalable learning-based framework} for dMRI. Our proposed stochastic greedy method preserves the performance of  \cite{gozcu2017, gozcu2019rethinking} while reducing the computational burden by a factor close to $200$.  %for MRI, where they proposed a greedy method exploiting fully-sampled training data, which has the advantage of being practical, flexible, as well as theoretically grounded, and the proposed method achieves similar performances with the previously greedy method while using $180$ times fewer computations. 

%The principle behind the greedy method is the following: We start from an empty mask, compute how much adding each phase encode (horizontal line of points in Fourier space) separately to the mask increases the quality of the reconstruction over some training images with respect to a performance metric (e.g. PSNR), and pick the phase encode which maximizes it. We keep iterating on all phase encodes not yet added to the mask up to a maximal cost (e.g $30\%$ sampling rate). G\"ozc\"u's approach typically uses all of the phase encodes at each iteration, which does not generalize well to dMRI due to the larger dimension of the data. The proposed stochastic greedy algorithm solves this issue by exploiting a fraction of the phases encodes at each iteration, while achieving a similar reconstruction quality, but with a \textit{drastic runtime improvement}.

Numerical evidence shows that our framework can successfully find sampling patterns for a broad range of decoders, from k-t FOCUSS \cite{jung2009k} to ALOHA \cite{jin2016general}, outperforming state-of-the-art model-based sampling methods over nearly all sampling rates considered. %Although we focused on single-coil Cartesian dynamic dMRI in the present study, our method can readily be generalized to parallel imaging as well as non-Cartesian setups.

%\textit{Outline of the paper:} In Section \ref{sec:background}, we introduce the CS formulation for dMRI. In the following Section \ref{sec:learning}, we formalize the problem of finding an optimal sampling distribution, prove our main result and detail our proposed algorithm. Then, in Section \ref{sec:experiments}, we demonstrate the benefits of the scalable approach against the framework of \cite{gozcu2017}, and proceed to show the effectiveness of our method compared to the existing approaches on several \textit{in vivo} data sets. Conclusions are drawn in Section \ref{sec:conclusion}.



==> ICASSP_Scalable_MRI_arXiv copy/02-setup.tex <==
%!TEX root = ms.tex
\vspace{-4mm}
\section{Theory}\label{sec:background}\shortestskip
\vspace{-.3cm}

\subsection{Signal Acquisition} \label{sec:pbm}
In the compressed sensing (CS) problem \cite{donoho2006compressed}, one desires to retrieve a signal that is known to be sparse in some basis using only a small number of linear measurements. In the case of dynamic MRI, we consider a signal $\*x \in \mathbb{C}^{p} = \mathbb{C}^{N^2 T}$ (i.e. a vectorized video of size $N\times N$ with $T$ frames), and the subsampled Fourier measurements are \useshortskip
\begin{equation}
\*b = \*P_{\Omega}\*{\Psi} \*x + \*w \label{eq:samp}
\end{equation}
where $\*{\Psi} \in \mathbb{C}^{p}$ is the spatial Fourier transform operator applied to the vectorized signal, $\*P_{\Omega} : \mathbb{C}^{p} \to \mathbb{C}^{n}$ is a subsampling operator that  
selects the rows of $\*\Psi$ according to the indices in the set $\Omega$ with $|\Omega| = n$ and $n \ll p$. We refer to $\Omega$ as \textit{sampling pattern} or \textit{mask}. We assume the signal $\*x$ to be sparse in the basis $\*\Phi$, which typically is a temporal Fourier transform across frames. Given the samples $\*b$, along with $\Omega$, a \textit{reconstruction algorithm} or \textit{decoder} $g$ forms an estimate $\*{\hat{x}}  = g(\*b, \Omega) $ of $\*x$.

The quality of the reconstruction is then evaluated using a \textit{performance metric} $\eta(\*x,\bm{\hat{\*x}})$, which could typically include Peak Signal-to-Noise Ratio (PSNR), the negative Mean Square Error (MSE), or the Structural Similarity Index Measure (SSIM) \cite{wang2004image}. 

\vspace{-.5cm}
\subsection{Sampling mask design}
\vspace{-.2cm}

We model the mask designing process as finding a probability mass function (PMF) $f \in S^{p-1}$, where $S^{p-1} := \{f \in [0,1]^p : \sum_{i=1}^p f_i =1\}$ is the standard simplex in $\mathbb{R}^p$. $f$ assigns to each location $i$ in the $k$-space a probability $f_i$ to be acquired. The mask is then constructed by drawing without replacement from $f$ until the cardinality constraint $|\Omega|=n$ is met. The problem of finding the optimal sampling distribution is subsequently formulated as \useshortskip
\begin{equation}
\max_{f\in S^{p-1}} \ef, % \mathbb{E}_{\Omega_f,X}\left[\eta\left(\*x, \*{\hat{x}}\left(\Omega,x\right)\right)\right] 
\qquad \ef :=  \mathbb{E}_{\substack{\Omega(f,n)\\ \*x \sim \mathcal{P}_{\*x}}}\left[\eta\left(\*x, \*{\hat{x}}\left(\Omega,\*x\right)\right)\right],
\label{eq:main}
\end{equation}
where the index set $\Omega\subset [p] $ is generated from $f$ and $[p] := \{1,\ldots,p\}$. This problem corresponds to finding the probability distribution $f$ that maximizes the expected performance metric with respect to the data $\mathcal{P}_{\*x}$ and the masks drawn from this distribution. To ease the notation, we will use $\eta\left(\*x, \*{\hat{x}}\left(\Omega,\*x\right)\right) \equiv \eta\left(\*x; \Omega\right)$.

%The relationship between $\eta$ and $H$ above is 
%\begin{align}
%H(f) & = \mathbb{E}_{\Omega_f,X}\left[ \eta\left(\*x, \*{\hat{x}}\left(\Omega,x\right)\right)\right] \nonumber\\
%& = \sum_{|\Omega|= n} \mathbb{E}_X\left[\eta\left(\*x, \*{\hat{x}}\left(\Omega,x\right)\right)\right] \Pr[\Omega] \nonumber\\
%& =  \sum_{|\Omega|=n} \mathbb{E}_X\left[\eta\left(\*x, \*{\hat{x}}\left(\Omega,x\right)\right)\right] \cdot  \frac{\prod_{k=1}^{m}  f_{\omega_k}}{ \prod_{k'=1}^{m-1} (1-\sum_{k=1}^{k'} f_{\omega_k})},
%\end{align}
%where the sums above are over all possible ordered index sets $\Omega = \{\omega_1,\cdots ,\omega_n\} \subset [p]$. 

In practice, we do not have access to $\mathbb{E}_{\mathcal{P}_{\*x}} \left[\eta(\*x; \Omega)\right]$ and instead have at hand the training images $\{\*x_i\}_{i=1}^m$ drawn independently from $\mathcal{P}_{\*x}$. We therefore maximize the empirical perfromance by solving \useshortskip
\begin{equation}
\label{eq:emp}
\max_{f\in S^{p-1}}  \emf, \text{~~~~} \emf :=\frac{1}{m} \sum_{i=1}^m \mathbb{E}_{\Omega(f,n)}\left[\eta(\Omega,\*x_i)\right].
 \end{equation}\useshortskip 
%where \useshortskip
%\begin{align}
%\emf  %:=& \sum_{|\Omega|=n}\frac{1}{m} \sum_{i=1}^m  \eta\l(  \Omega ,\*x_i\r) \cdot  \Pr[\Omega|f]
% \nonumber\\
%:=&\frac{1}{m} \sum_{i=1}^m \mathbb{E}_{\Omega(f,n)}\left[\eta(\Omega,\*x_i)\right].
%\end{align}
Given that Problem \eqref{eq:emp} looks for  masks that are constructed by sampling $n$ times without replacement from $f$, the following holds.
\begin{proposition}
There exists a maximizer of Problem \eqref{eq:emp} that is supported on an index set of size at most $n$.\label{prop:1}
\end{proposition}
\begin{proof}
Let the distribution $\widehat{f}_n$ be a maximizer of Problem~\eqref{eq:emp}. We are interested in finding the support of $\widehat{f}_n$. Because $\sum_{|\Omega|=n}\Pr[\Omega]=1$, note that 

\begin{align}
\max_{f\in S^{p-1}}  \emf & := \max_{f\in S^{p-1}}  \sum_{|\Omega|=n}  \frac{1}{m}\sum\nolimits_{i=1}^m\eta(\*x_{i};\Omega) \cdot \Pr[\Omega|f]\nonumber\\ 
& \le \max_{f\in S^{p-1}} \max_{|\Omega|=n} \frac{1}{m}\sum\nolimits_{i=1}^m\eta(\*x_{i}; \Omega) \nonumber\\
& = \max_{|\Omega|=n}   \frac{1}{m}\sum\nolimits_{i=1}^m\eta(\*x_{i};\Omega). 
\end{align}
Let $\widehat{\Omega}_n$ be an index set of size $n$ that maximizes the last line above. 
The above holds with equality when $\Pr[\widehat{\Omega}_n]=1$ and $\Pr[\Omega]=0$ for $\Omega\ne \widehat{\Omega}_n$ and $f=\widehat{f}_n$. This in turn happens when $\widehat{f}_n$ is  supported on $\widehat{\Omega}$. That is, there exists a maximizer of Problem \eqref{eq:emp} that is supported on an index set of size $n$. 
\end{proof}
While this observation does not indicate how to find this maximizer, it nonetheless allows us to further simplify Problem \eqref{eq:emp}. More specifically, the observation that a distribution $\widehat{f}_n$ has a compact support of size $n$ implies the following:
\begin{proposition}\useshortskip
\begin{equation}
\text{Problem \eqref{eq:emp}} \equiv  \max_{|\Omega|=n}  \frac{1}{m}\sum_{i=1}^m \eta(\*x_{i}; \Omega) \label{eq:greedy}
\end{equation} \label{prop:2}
\vspace{-.5cm}
\end{proposition}
\begin{proof}
Proposition~\ref{prop:1} tells us that a solution of Problem~\eqref{eq:emp} is supported on a set of size at most $n$, which implies
\begin{equation}
\text{Problem \eqref{eq:emp}} \equiv 
\max_{f\in S^{p-1}, |\text{supp}(f)| = n }\emf\label{eq:main emp equiv 1}.
\end{equation} 
That is, we only need to search over compactly supported distributions $f$. Let $S_\Gamma$ denote the standard simplex on a support $\Gamma\subset [p]$. It holds that
\begin{align}
\text{Problem \eqref{eq:main emp equiv 1}} &  \equiv
\max_{|\Gamma|=n} \max_{f\in S_\Gamma}\emf \nonumber\\
% = \max_{|\Gamma|=n} &\max_{f\in S_\Gamma} \sum_{|\Omega|=n}\frac{1}{m}\sum\nolimits_{i=1}^m\eta(\*x_{i};\Omega) \cdot \Pr[\Omega|f] \nonumber\\
 = \max_{|\Gamma|=n} &\max_{f \in S_\Gamma} \frac{1}{m}\sum\nolimits_{i=1}^m\eta(\*x_{i};\Gamma) \cdot \Pr[\Gamma|f] \nonumber\\
 = \max_{|\Gamma|=n}& \max_{f \in S_\Gamma} \frac{1}{m}\sum\nolimits_{i=1}^m\eta(\*x_{i};\Gamma) \nonumber\\
 =  \max_{|\Gamma|=n} & \frac{1}{m}\sum\nolimits_{i=1}^m\eta(\*x_{i};\Gamma).
\label{eq:main emp equiv 2}
\end{align}
To obtain the second and third equalities, one observes that all masks have a common support $\Gamma$ with $n$ elements, i.e. $f\in S_\Gamma$ allows only for a single mask $\Omega$ with  $n$ elements, namely $\Omega=\Gamma$.~\end{proof}
%As $\Omega$ is obtained by sampling $n$ times without repetition from $f$, then $\Omega = \Gamma$ after $n$ draws, so $\Pr[\Gamma|f]=1$%the all masks all be contained on the same support $\Gamma$, which means that in the end, a single mask supported on~$\Gamma$ will be obtained with $\Pr[\Gamma]=1$.
%which is exactly the formulation of equation \eqref{eq:erm}, which means that trying to learn an optimal support is equivalent to trying to learn the optimal sampling distribution.
The framework of Problem~\eqref{eq:emp} captures most variable-density based approaches of the literature that are defined in a data-driven fashion \cite{seeger2010optimization,ravishankar2011adaptive,vellagoundar2015robust,weizman2015compressed,haldar2019oedipus,bahadir2019learning,sherry2019learning}, and Proposition \ref{prop:2} shows that Problem~\eqref{eq:main emp equiv 2}, that we tackled in \cite{gozcu2017,gozcu2019rethinking} and develop here, also aims at solving the \textit{same} problem as these probabilistic approaches. 
Note that while the present theory considered sampling \textit{points} in the Fourier space, it is readily applicable to the Cartesian case, where full lines are added to the mask at once. %generalizable to adding full lines to the mask,  

%Many reconstructions have been proposed over the years, and we detail hereafter several state of the art methods that are considered in Section~\ref{sec:experiments} for single-coil datasets. An early approach for successful CS recovery in dynamic MRI is k-t FOCUSS \cite{jung2009k}, which approximates the result of the problem 
% \begin{equation} 
%\underset{\*x\in\mathbb{C}^p}{\text{max}} \| \*\Phi \*x\|_1 \text{ s.t. }  \| \*P_\Omega \*\Psi\*x - \*b \|_2 \leq\epsilon \label{eq:l1}.
%\end{equation}
% A later method is the Iterative Soft-Thresholding (IST), which directly solves the problem \eqref{eq:l1} \cite{otazo2012combination}. More recently, a generic framework for both single and multi-coil dMRI was developed named annihilating filter based low-rank Hankel matrix approach (ALOHA) by Jin et al. \cite{jin2016general}. ALOHA exploits the duality between sparse signals and their transform domain representations cast as a low-rank Hankel matrix. This duality can be used to reformulate the CS recovery as a low-rank matrix completion problem.
% 
% 
%Many other algorithms have been developed to solve the dynamic MRI problem with Cartesian sampling, and the first one to be used was k-t SPARSE \cite{lustig2006kt}, which solves the problem \eqref{eq:l1} with a conjugate gradient method.  Other approaches combined low-rank and sparse approaches \cite{lingala2011accelerated,tremoulheac2014dynamic, otazo2015low}, or use dictionary learning to sparsely represent a signal \cite{ravishankar2011mr,wang2014compressed, caballero2014dictionary}, and more recently, deep learning reconstructions \cite{schlemper2018deep} have yielded promising results. While we primarily consider Cartesian dMRI here, non-Cartesian sampling based on radial trajectories has also been used broadly to enable free-breathing scans  \cite{feng2014golden,feng2016xd}. 
%
%\vspace{-3mm}

%\subsection{Sampling mask design}
%The most widely used approach for the design of the sampling pattern $\*\Omega$ is \textit{random variable-density sampling}, which was originally proposed by Lustig et al. \cite{lustig2007sparse} for static MRI and adapted to dynamic MRI by Jung et al. \cite{jung2007improved}. It offers a compromise between incoherent measurements, required by the theory of CS, and the structure that can be found in the \mbox{k-space}, where most of the energy is concentrated in the low frequency end of the spectrum. This classical approach draws random samples according to a parametric distribution mimicking the energy distribution of the \mbox{k-space}, favoring low-frequency samples. The distribution considered is typically either polynomial \cite{lustig2007sparse, kim2012accelerated, tremoulheac2014dynamic, weizman2015compressed}, or Gaussian \cite{jung2009k, otazo2010combination, caballero2014dictionary,otazo2015low,jin2016general,schlemper2018deep}. In these setups, a slight offset is often added in order to prevent the distribution from having extremely small probabilities at high-frequencies, and a few low-frequency \mbox{k-space} samples are acquired at the Nyquist rate.
%
%The variable-density based methods commonly used in dMRI perform well, but have several weaknesses, already highlighted in \cite{gozcu2017} for static MRI. They require parameters to be tuned, such as decay rate of the polynomial, the standard deviation of the Gaussian distribution or the number of central phase encodes and arbitrarily constrain the sampling patterns to a model without any theoretical justification. Moreover, it is unclear which sampling density will be most effective for a given anatomy and reconstruction rule. Also, the idea of randomizing the acquisition is in itself questionable, as in practice, one would desire to design a fixed sampling pattern that we will know to perform well for a specific anatomy across many subjects. Finally, some variable-density methods, such as Poisson Disc Sampling \cite{vasanawala2011practical}, do not use a fixed number of readouts per frame, which complicates their hardware implementation for dynamic MRI \cite{ahmad2015variable}. Indeed, undersampling some frames more heavily than others might result in missing critical temporal information.
%
%Recently, several articles have focused on improved design of spatiotemporal sampling patterns for dMRI, and we hereafter detail two particularly relevant methods. A recent state-of-the-art method devised for this purpose is the variable density incoherent spatiotemporal acquisition (VISTA) \cite{ahmad2015variable} that maximizes Riesz energy on a spatiotemporal grid, and has the notable advantage of generating patterns with high levels of incoherence, and maintaining uniform sampling density across frames. Another important technique proposed by Li et al. \cite{li2018dynamic} develops a method for Cartesian sampling exploiting the golden-ratio, with the aim to generate incoherent measurements and maintain uniform sampling density across frames\footnote{This approach is different from the commonly used golden-\textit{angle} sampling used in radial sampling.}. 
%
%Other relevant undersampling works include, in the non-Cartesian  setting, fully random radial sampling \cite{jung2010radial, tremoulheac2014dynamic}, as well as golden-angle radial sampling,  where spokes separated by the golden-angle are continuously acquired \cite{winkelmann2007optimal, feng2014golden,feng2016xd}. These results exploit the inherent advantage of radial over Cartesian sampling that each spoke goes through the sample of the k-space and can thus contain low-frequency as well as high-frequency information. More recent work also leverage variable-density approaches in the non-Cartesian setting \cite{boyer2016generation,lazarus2018variable} Also, in static MRI, several methods exploiting training signals have been proposed: in \cite{knoll2011adapted, zhang2014energy,vellagoundar2015robust}, a distribution from which random samples are drawn is constructed, and in \cite{seeger2010optimization,ravishankar2011adaptive,liu2012under, haldar2019oedipus}, a single image is used at a time to determaxe the sampling mask. Very recently, deep-learning based methods have enabled active mask design paired with online reconstruction and shown very promising results \cite{jin2019self,zhang2019reducing,weiss2019learning}. However, to the best of our knowledge, none of these methods have been extended to dynamic MRI. 

%\subsection{Our contributions}
%In this paper, we extend the \textit{learning-based framework} of G\"ozc\"u et al. \cite{gozcu2017} for efficiently designing sampling masks based on empirical risk maximization. We preserve the benefits of this recent approach against the state-of-the-art mask design methods, as we do not set any assumptions on the structure of signal, but consider the samples to come from an unknown probability distribution. Both methods are tailored to the anatomy and the reconstruction algorithm at hand, allow direct optimization for a given performance measure and are highly parallelizable. Our scalable version extends this previous work in the following ways
%\begin{itemize}[leftmargin=*]
%\item We propose a scalable version of the greedy algorithm of \cite {gozcu2017}, which achieves similar reconstruction accuracy by using up to $60$ times less resources. This is achieved by implementing a stochastic greedy method.
%\item This enables a successful extension of this framework to dynamic MRI, where the approach of G\"ozc\"u et al. is not computationally \rev{feasible.}
%%\item Due to the significant reduction of the computational burden with our algorithm, we anticipate its successful application to parallel imaging, where the reconstructions are slower, as well as to 3D (d)MRI.
%\item Our algorithm allows for keeping the number of samples per frame to be constant, in order for the effective acceleration in scan time to be the consistent with the undersampling rate. This design constraint does not add any computational burden and results from the flexibility of this framework. 
%\item We empirically show the improvement of our method over the state-of-the-art mask designs and several model-based reconstruction algorithms on \textit{in vivo} datasets. 
%\item \rev{Finally, given a fixed computational budget, we provide a thorough comparison between our data-driven approach and the model-based approach of tuning parameters of \textit{a priori} assumed distribution to optimize reconstruction quality. We show that our model-free method consistently outperforms this state-of-the-art approach.}
%%\item \rev{Also, we show that, given a fixed computational budget, optimizing the parameters of parametric distributions via usual parameter sweeps, is consistently outperformed by our model-free method.}



%\end{itemize}


==> ICASSP_Scalable_MRI_arXiv copy/03-algo.tex <==
%!TEX root = ms.tex
\vspace{-.3cm}
\section{Stochastic greedy mask design}\label{sec:learning}
\vspace{-.3cm}
Aligned with the approach that we previously proposed in \cite{gozcu2017}, we want to find an approximate solution to Problem~\eqref{eq:greedy} by leveraging a greedy algorithm. This is required by Problem~\eqref{eq:greedy} being inherently combinatorial. The previous greedy method of \cite{gozcu2017,gozcu2019rethinking} suffers from three main drawbacks: \di it scales quadratically with the total number of lines, \ii it scales linearly with the size of the dataset, and \iii it does not construct mask with a fixed number of readouts by frame. While \cite{gozcu2019rethinking} partially deals with \textbf{(i)}, our proposed stochastic greedy approach addresses all three issues, while preserving the benefits of \cite{gozcu2017}. It notably still preserves the nestedness and ordering of the acquisition, where critical locations are acquired initially, and the mask built outputs a nested structure (i.e. the mask at $30\%$ sampling rate includes all sampling locations of the mask at $20\%$).

Let us introduce the set $\mathcal S$ of all lines that can be acquired, which is a set of subsets of $\{1,\dotsc,p\}$. A feasible Cartesian mask takes the form $ \Omega = \bigcup_{j=1}^\ell S_j, \quad S_j \in \mathcal{S}$, i.e. it consists of a union of lines.  Both the greedy method of \cite{gozcu2017} and our stochastic method are detailed in Algorithm \ref{alg:1} below. Our stochastic greedy method (\textbf{SG-v2}) addresses the three main limitations of the greedy method of \cite{gozcu2017} (\textbf{G-v1}).  The issue \di is solved by picking uniformly at random  at each iteration a batch possible lines $\mathcal{S}_{iter}$ of size $k$  from a given frame $\mathcal{S}_t$, instead of considering the full set of possible lines $\mathcal{S}$ (line 3 in Alg. \ref{alg:1}); \ii is addressed by considering  a fixed batch of training data $\mathcal{L}$ of size $l$ instead of the whole training set of size $m$ at each iteration (line 4 in Alg. \ref{alg:1}); \iii is solved by iterating through the lines to be added from each frame $\mathcal{S}_t$ sequentially (lines 1, 3 and 10 in Alg. \ref{alg:1}).  These improvements are inspired by the refinements done to the standard greedy algorithm in the field of submodular optimization \cite{mirzasoleiman2015lazier}, and allow to move the computational complexity from $\Theta\left(mr(NT)^2\right)$ to $\Theta\left(lrkNT\right)$, effectively speeding up the computation by a factor $\mathbf{\Theta(\frac{m}{l}\frac{NT}{k})}$. Our results show that this is achieved without sacrificing any reconstruction quality.\vspace{-.2cm}


%
%
%In the compressed sensing (CS) problem \cite{donoho2006compressed}, one desires to retrieve a signal that is known to be sparse in some basis using only a small number of linear measurements. In the case of dynamic MRI, we consider a signal $\*x \in \mathbb{C}^{N\times N\times T}$ (i.e. a video of size $N\times N$ with $T$ frames), which will be written on a vectorized form $\*x \in \mathbb{C}^{p}$ for convenience, and we have subsampled Fourier measurements described as
%
%\begin{equation}
%\*b = \*P_{\Omega}\*{\Psi} \*x + \*w \label{eq:samp}
%\end{equation}
%where $\*{\Psi} \in \mathbb{C}^{p}$ is the spatial Fourier transform operator applied to the vectorized signal, $\*P_{\Omega} : \mathbb{C}^{p} \to \mathbb{C}^{n}$ is a subsampling operator that  
%selects the rows of $\*\Psi$ according to the indices in the set $\*\Omega$ with $|\Omega| = n$ and $n \ll p$. We refer to $\Omega$ as \textit{sampling pattern} or \textit{mask}. Given the samples $\*b$, along with $\Omega$, a \textit{reconstruction algorithm} or \textit{decoder} $g$ then forms an estimate $\*{\hat{x}}$ of $\*x$ such that
%\begin{equation}
%	\*{\hat{x}} := g(\Omega,\*b) = g(\Omega,\*x).
%\end{equation}
%The quality of the reconstruction is then evaluated using a \textit{performance metric} $\eta(\*x,\bm{\hat{\*x}})$, which could typically include Peak Signal-to-Noise Ratio (PSNR), the negative Mean Square Error (MSE), or the Structural Similarity Index Measure (SSIM) \cite{wang2004image}. 


%Acquisition modelling

%Procedure of acquisition: sequential, growing mask



%An algorithm performing mask optimization should address two important design constaints:
%\begin{enumerate}
%\item \textbf{Nestedness:} as the phase encoding lines are sequentially acquired during a mask, the algorithm should output a nested structure. A mask at $30\%$ sampling rate should include all sampling locations of the mask at $20\%$.
%\item \textbf{Ordering:} locations which critically improve the performance should be favoured.
%\end{enumerate} 


%In accelerated Cartesian MRI, phase encoding line are sequentially acquired and the k-space is gradually filled until the desired undersampling ratio is reached. The mask $\Omega$ should first of all be constructed to include union of lines in the k-space to satisfy this design constraints. To formalize this, we define a set $\mathcal S$ of subsets of $\{1,\dotsc,p\}$ which typically contains phase encoding lines in the k-space. The final mask then takes the form 
%\begin{equation}
 %   \Omega = \bigcup_{j=1}^\ell S_j, \quad S_j \in \mathcal{S}
%\end{equation}
%for some $\ell> 0$.  It 

%Assume now that we are given a set of training samples $\*x_{1}, \dotsc,\*x_{m}\in \mathbb{C}^{N\times N\times T}$  representative of an unknown signal of interest $\*x$. Formally, the samples are independently drawn from the same unknown probability distribution $X \subset \mathbb{C}^{p}$. 
%The mask $\Omega$ is typically constructed as draw from a probability distribution $f\in [0,1]^p$, where $f_{i}$ is the probability of the i  %\c % which assigns $1$ to a location $(i,j)$ with probability
%The question of sampling optimization in MRI revolves around finding a g

%We assume the signal $\*x$ to be sparse in the basis $\*\Phi$, which typically is a temporal Fourier transform across frames \cite{jung2009k, otazo2012combination, feng2014golden, tremoulheac2014dynamic, otazo2015low,jin2016general,schlemper2018deep}. Given the samples $\*b$, along with $\Omega$, a \textit{reconstruction algorithm} or \textit{decoder} $g$ forms an estimate $\*{\hat{x}}$ of $\*x$ such that
%\begin{equation}
%\*{\hat{x}} = g(\*b, \Omega)
%\end{equation}



%\subsection{Model-free approach}
%Our work follows the learning-based framework of \cite{gozcu2017}, and we summarize their main ideas hereafter. We assume that we have a set of training samples $\*x_{1}, \dotsc,\*x_{m}\in \mathbb{C}^{N\times N\times T}$  representative of an unknown signal of interest $\*x$. This means that they are all drawn from the same unknown probability distribution $X \subset \mathbb{C}^{p}$, with the  corresponding probability space $(X,B_X,\mu)$, where $B_X$ is the (subspace) Borel sigma algebra on $X$, and $\mu$ is a probability measure. We are concerned here by the noiseless case, i.e. $\*w = 0$, and the noisy case is covered in Section 4 of the Supplementary Material.


%We wish to find the sampling pattern $\Omega^{*}$ that will perform best on $\*x$, according to some \textit{performance metric} $\eta(\*x,\bm{\hat{\*x}})$, and  given some constraints on the design of the mask.  A performance metric enables quantification of the similarity of a reconstructed image to the ground truth, and common metrics include Peak Signal-to-Noise Ratio (PSNR), Mean Square Error (MSE) and Structural Similarity Index Measure (SSIM) \cite{wang2004image}. 
%Regarding the constraints on $\Omega$, it is desirable to restrict the sampling pattern to contain for instance only horizontal and/or vertical phase encoding directions. To formalize this, we define a set $\mathcal S$ of subsets of $\{1,\dotsc,p\}$ which typically contains phase encoding lines in the k-space. The final mask then takes the form 
%\begin{equation}
%    \Omega = \bigcup_{j=1}^\ell S_j, \quad S_j \in \mathcal{S}
%\end{equation}
%for some $\ell> 0$. In the present work, we only focus on imposing a cardinality constraint to each mask, i.e. a constraint on the sampling rate. We assume that the final mask must satisfy $|\Omega| \le n$, where $n$ is equal to the number of points that can be acquired.  This then leads to the problem of finding the mask that maximizes
%\begin{equation}
%\Omega^{*} = \underset{\Omega \in \mathcal A}{\text{arg max }} \mathbb E_{X} \left[\eta(\*x,{\hat{\*x}})\right] \label{eq:expec}
%\end{equation}
%where $\mathcal A$ is the set of feasible $\Omega$ according to $\mathcal S$ and $n$. Due to the problem \eqref{eq:expec} not being tractable in practice, we look for an approximate maximizer in the form of the {\em empirical average}, which yields the selection rule that will be used in the sequel
%\begin{equation}
%    \hat{\Omega} = \argmax_{\Omega \in \mathcal{A}} \frac{1}{m} \sum_{j=1}^m \eta(\*x_j,\hat{\*x}_{j}). \label{eq:erm}
%\end{equation}
%
%Given that enough training samples are considered, statistical learning theory guarantees that the result obtained using the empirical average will be close to the true average, and Proposition 1 of \cite{gozcu2017}, which formalizes and proves this, extends to the present case as well.
%
%\subsubsection{Finding the optimal sampling distribution}
%
%Let also $f\in [0,1]^{p}$ be a probability distribution on the pixels, where $p_{i}$ is the probability of sampling the $i$th pixel of $\*\Psi\*x 
%$.  Note that $f\in S_{n}$, where $S_n$ is the standard simplex in $\R^{n}$.  $\Omega$ is then constructed by sampling $n$ times without replacement from $f$. The problem of finding the optimal sampling distribution is then formulated as 
%\begin{equation}
%\max_{f\in S_{n}} H(f), % \mathbb{E}_{\Omega_f,X}\left[\eta\left(\*x, \*{\hat{x}}\left(\Omega,x\right)\right)\right] 
%\qquad  H(f) :=  \mathbb{E}_{\Omega_f,X}\left[\eta\left(\*x, \*{\hat{x}}\left(\Omega,x\right)\right)\right]
%\label{eq:main}
%\end{equation}
%where the index set $\Omega\subset [p]$ is generated from $f$. 
%Given a probability distribution $f$ and a cardinality constraint $n$

% \begin{equation}\left
 %\Omega =\{\omega_1,\cdots,\omega_n\}  \subset [p]
 %\end{equation}
%by sampling $n$ times from this distribution (without  replacement).  
%For $\*x\in X$ and an index set $\Omega$, consider the $n$ measurement vector $\*P_\Omega \*\Psi\*x \in \mathbb{C}^{n}$ obtained by setting to zero all entries not indexed in $\Omega$. That is, $P_\Omega Fx$ is the orthogonal projection of $Fx$ onto the index set $\Omega$. 
%Given the measurement matrix  $b=\*P_\Omega \*\Psi\*x$ and decoder $\Delta$, we recover $\Delta(\Omega,b)=\Delta(\Omega,x)$ and incur the loss $g(x,\Delta(\Omega,x)) = g(\Omega,x)$. 
%For this decoder, we would like to learn the best distribution $p$ by solving the Problem 

% Let $p^-$ be the sequence obtained from $p$ by removing its last entry $p_{n,n}$. Note  that 
%\begin{equation}
%p\in S_{n,n} \Longrightarrow p^-\in S^-_{n,n} =\l \{ p' : \sum_{[i,j]\ne [n,n]} p'_{i,j}\le 1,\quad p'_{i,j}\ge 0\r\}. 
%\end{equation}
%The relationship between $\eta$ and $H$ above is 
%\begin{align}
%H(f) & = \mathbb{E}_{\Omega_f,X}\left[ \eta\left(\*x, \*{\hat{x}}\left(\Omega,x\right)\right)\right] \nonumber\\
%& = \sum_{|\Omega|= n} \mathbb{E}_X\left[\eta\left(\*x, \*{\hat{x}}\left(\Omega,x\right)\right)\right] \Pr[\Omega] \nonumber\\
%& =  \sum_{|\Omega|=n} \mathbb{E}_X\left[\eta\left(\*x, \*{\hat{x}}\left(\Omega,x\right)\right)\right] \cdot  \frac{\prod_{k=1}^{m}  f_{\omega_k}}{ \prod_{k'=1}^{m-1} (1-\sum_{k=1}^{k'} f_{\omega_k})},
%\end{align}
%where the sums above are over all possible ordered index sets $\Omega = \{\omega_1,\cdots ,\omega_n\} \subset [p]$. 
%Consider the change of variables $q_{i,j}=\log p_{i,j}$ for all $i,j$, under which the objective function of Problem \eqref{eq:main} becomes convex, namely
%\begin{equation}
%\sum_{|\Omega|=m} \mathbb{E}_x g \l(  \Omega ,x\r) \cdot  \frac{\prod_{k=1}^{m}  e^{\sum_{k=1}^m q_{\omega_k}} }{ \prod_{k'=1}^{m-1} (1-\sum_{k=1}^{k'} e^{q_{\omega_k}}) } 
%\end{equation}
%is a convex function of $q$. Indeed, note that 
%\begin{align}
%&  \log\l( \frac{\prod_{k=1}^{m}  e^{\sum_{k=1}^m q_{\omega_k}} }{ \prod_{k'=1}^{m-1} (1-\sum_{k=1}^{k'} e^{q_{\omega_k}}) } \r) \nonumber\\
%& = \sum_{k=1}^m q_{\omega_k} - \log\l( 1-e^{q_{\omega_1}} \r)\cdots  - \log\l(
%1-\sum_{ k=1}^{m-1} e^{q_{\omega_{k}}} \r),
%\end{align}
%and it is not difficult to verify that each logarithmic term above is concave.  Under this change of variables, Problem \eqref{eq:main} is equivalent to 
%\begin{equation}
%\begin{cases}
%\min_q  G_g(q)\\
%\sum_{i,j=1}^n e^{q_{i,j}} = 1,
%\end{cases}
%\qquad  G_g(q) = 
%\sum_{|\Omega|=m} \mathbb{E}_x f(\Omega,x) \cdot 
%\frac{\prod_{k=1}^{m}  e^{\sum_{k=1}^m q_{\omega_k}} }{ \prod_{k'=1}^{m-1} (1-\sum_{k=1}^{k'} e^{q_{\omega_k}}) }. 
%\end{equation} 
%In practice, we don't have access to $\mathbb{E}_X \eta(\Omega,x)$ and instead have at hand the training images $x_{1:m}=\{x_l\}_{l=1}^m$ drawn independently from $X$. We therefore minimize the empirical risk by solving  
%\begin{equation}
%\label{eq:emp}
%\min_{f\in S_{n\times n}}  H_m(f),
%\end{equation} 
%where 
%\begin{align}
% H_m(f)  & =
% \sum_{|\Omega|=n} \eta(\Omega,x_{1:m}) \cdot \Pr[\Omega] \nonumber\\
%& := \sum_{|\Omega|=n}\frac{1}{m} \sum_{l=1}^m  \eta\l(  \Omega ,x_l\r) \cdot  \Pr[\Omega]
% \nonumber\\
%& =\frac{1}{m} \sum_{l=1}^m \mathbb{E}_{\Omega} \eta(\Omega,x_l).
%\end{align}

%\subsubsection{Support}

%Let the distribution $\widehat{f}_m$ be a minimizer of Problem \eqref{eq:emp}. We are interested in finding the support of $\widehat{f}_m$. Because $\sum_{|\Omega|=n}\Pr[\Omega]=1$, note that 
%\begin{align}
%\min_{f\in S_{n}}  \sum_{|\Omega|=n}  \eta(\Omega,x_{1:m}) \cdot \Pr[\Omega] & \ge 
%\min_{f\in S_{n}} \min_{|\Omega|=n} \eta(\Omega,x_{1:m}) \nonumber\\
%& = \min_{|\Omega|=n}  \eta(\Omega,x_{1:m}). 
%\end{align}
%Let $\widehat{\Omega}_m$ be an index set of size $n$ that minimizes the last line above. 
%Above holds with equality when $\Pr[\widehat{\Omega}_m]=1$ and $\Pr[\Omega]=0$ for $\Omega\ne \widehat{\Omega}_m$ for $f=\widehat{f}_s$. This in turn happens when $\widehat{f}_s$ is  supported on $\widehat{\Omega}$. That is, there exists a minimizer of Problem \eqref{eq:emp} that is supported on an index set of size $n$. 
%
%This observation allows us to further simplify Problem \eqref{eq:emp}. More specifically, the observation that an optimal distribution $\widehat{p}_s$ has a compact support of size $m$ implies that 
%\begin{align}
%\text{Problem \eqref{eq:emp}} \equiv 
%\begin{cases}
%\min_{f\in S_{n\times n}} H_m(f) \\
%|\text{support}(f)| = n.
%\end{cases}
%\label{eq:main emp equiv 1}
%\end{align}
%That is, we only need to search over compactly supported distributions $F$. In turn, if $S_\Gamma$ denotes the standard simplex on a support $\Gamma\subset [p]$, we have that 
%\begin{align}
%\text{Problem \eqref{eq:main emp equiv 1}} &  \equiv
%\min_{|\Gamma|=n} \min_{f\in S_\Gamma} G_m(f) \nonumber\\
%& = \min_{|\Gamma|=n} \min_{f\in S_\Gamma} \sum_{|\Omega|=m} \eta(\Omega,x_{1:m}) \cdot \Pr[\Omega] \nonumber\\
%& = \min_{|\Gamma|=n} \min_{f \in S_\Gamma} \eta(\Gamma,x_{1:m}) \cdot \Pr[\Gamma] \nonumber\\
%& = \min_{|\Gamma|=n} \min_{f \in S_\Gamma} \eta(\Gamma,x_{1:m}) \nonumber\\
%& = \min_{|\Gamma|=n}g(\Gamma,x_{1:m}),
%\label{eq:main emp equiv 2}
%\end{align}
%which is exactly the formulation of equation \eqref{eq:erm}, which means that trying to learn an optimal support is equivalent to trying to learn the optimal sampling distribution.%, that is, the optimization solved in that paper to learn the optimal support was theoretically well-justified. 

%\subsubsection{Greedy algorithm}
%Before moving on to our stochastic greedy method, we describe the straightforward application of G\"ozc\"u's framework to dMRI. Because finding the exact maximizer of \eqref{eq:erm} is difficult in general, the greedy algorithm proposed by G\"ozc\"u et al. \cite{gozcu2017} finds an approximate solution by exploiting the fact that the generalization bound dictates that a mask with improved performance should always be favored. This greedy approach has the advantage over state-of-the-art methods of being parameter free in the sense that no tuning is required for the mask selection process, once the reconstruction algorithm and its parameters are given. 
%
%The details are specified in Algorithm \ref{alg:1}. We start from a base mask $\Omega$, and at each iteration, we create candidate masks $\Omega' = \Omega \cup S$ with each subset $ S \in \mathcal{S}$ not yet included in the mask $\Omega$. After reconstructing the image ${\hat{\*x}}$ in the training dataset using the decoder $g$ for all the $\Omega'$, the subset $S$ that yields the larger increase regarding the performance metric $\eta$ is permanently added to the mask $\Omega$. The algorithm continues to add subsets from $\mathcal{S}$ while the cost constraint $\Gamma$ is not violated. This is what 

%\begin{figure}[!t]
%\centering
%\includegraphics[width=.9\linewidth,valign=t]{figures/schema2}
%\caption{ Illustration of two iterations of Algorithm \ref{alg:1}, the evaluation of $\eta(\Omega)$ is explicited on the right figure.}\label{fig:schema}
%\end{figure}

%The algorithm also exhibits a useful \textit{nestedness} property, which means that both the order in which the samples are added to the mask and their cost are known. Once a given cost is reached (e.g. $30\%$ sampling), all the masks for smaller costs remain available (e.g. the mask for $20\%$ sampling rate). However, there is a limited applicability of Algorithm \ref{alg:1}.a to dMRI that comes from the fact that the number of samples increases linearly with the number of frames, and that the reconstruction algorithms are generally more expensive to run than in the static case. This makes the overall running time of Algorithm \ref{alg:1}.a impractical for the present case, as we will see in Section \ref{sec:experiments}. We will refer to the framework of  \cite{gozcu2017} as \textbf{G-v1}.

%The properties of greedy algorithms have been well studied in the field of submodular optimization \cite{nemhauser1978analysis}, where they achieve near-optimal results. Submodularity denotes the idea of diminishing return: adding one phase encoding line to a mask with 10-fold undersampling will have more return than adding the same phase encoding line to a mask having 5-fold undersampling. The setting of our problem and its generic pairing with any reconstruction algorithm yields a the cost function \eqref{eq:erm} that cannot be written in a closed form, and prohibits a straigtforward analysis of this function to establish any form of submodularity in the general setting. However, while it is challenging to show that the present problem of sampling optimization in dynamic MRI is submodular, it still behaves similarly to submodular problems, especially regarding this property of diminishing returns, and this is why one can expect such an approach to exhibit good performance.

\begin{algorithm}[ht]
\caption{Greedy mask optimization algorithms for dMRI \\ \textbf{(G)} refers to the greedy algorithm \cite{gozcu2017} \\   \textbf{(SG)} refers to the \textbf{stochastic greedy} algorithm  \\ \textbf{(v1)}  algorithm iterated throughout the whole training set \\ \textbf{(v2)} algorithm iterated through batches of training examples}\label{alg:1}
\textbf{Input}: Training data $\{\*x\}_{i=1}^m$, recon. rule $g$, sampling set $\mathcal{S}$, max. cardinality $n$, samp. batch size $k$, train. batch size $l$ \\
\textbf{Output}: Sampling pattern $\Omega$
\begin{algorithmic}[1]
\State 
 \begin{tabular}{ccc} 
\textbf{(SG) }  Initialize $t=1$  
    \end{tabular}
 \While{$|\Omega| \leq n$}
        
        \State   $ \left \{\begin{tabular}{l}
 \textbf{(G)~~~} Pick $\mathcal{S}_{iter} = \mathcal{S}$   \\
 \textbf{(SG)~} Pick $\mathcal{S}_{iter}\subseteq \mathcal{S}_t$ at random, with $|\mathcal{S}_{iter}| = k$  
  \end{tabular} \right.$
        \State   $ \left \{\begin{tabular}{l}
 \textbf{(v1) } Pick $\mathcal{L} = \{1,\ldots,m\}  $ \\
 \textbf{(v2) } Pick $\mathcal{L} \subseteq \{1,\ldots,m\} $, with $|\mathcal{L}| = l $
  \end{tabular} \right.$
         \For{$S \in \mathcal{S}_{iter} \text{ such that } |\Omega \cup S| \leq \Gamma$} 
     
        \State  $\Omega' = \Omega \cup S$ 
        \State For each $\ell \in \mathcal{L}$ set ${\hat{\*x}}_\ell\leftarrow g(\Omega', \*P_{\Omega'}\bm\Psi\*x_\ell)$
%$\*b_\ell\leftarrow \*P_{\Omega'}\bm\Psi\*x_\ell$, ${\hat{\*x}}_\ell\leftarrow g(\Omega', \*P_{\Omega'}\bm\Psi\*x_\ell)$
        \State   $\eta(\Omega') \leftarrow \frac{1}{|\mathcal{L}|} \sum_{\ell\in\mathcal{L}} \eta(\*x_\ell, {\hat{\*x}}_\ell)$
 \EndFor
 \State $\displaystyle\Omega \leftarrow \Omega \cup S^*,  \text{ where }$   $\displaystyle S^* = \argmax_{\substack{S:|\Omega \cup S| \leq n}} \eta(\Omega\cup S)$
\State   \textbf{ (SG) }   $t= (t \bmod T)+1$  
    \EndWhile
\State {\bf return} $\Omega$ 
\end{algorithmic}

\end{algorithm} 
%\begin{algorithm}[ht]
%\caption{Greedy mask optimization algorithms for dMRI \\ \textbf{(G)} refers to the greedy algorithm \\   \textbf{(SG)} refers to the \textbf{Stochastic greedy} algorithm  \\  \textbf{(SCG)} refers to the \textbf{Stochastic cycling greedy} algorithm \\ \textbf{(v1)} refers to the version where the algorithm is iterated throughout the whole training set \\ \textbf{(v2)} refers to the version where the algorithm is iterated through a subset of the whole training set picked at random at each iteration}\label{alg:1}
%\textbf{Input}: Training data $\*x_1, \ldots, \*x_m$, reconstruction rule $g$, sampling subset $\mathcal{S}$, maximum cardinality $\Gamma$, sampling batch size $k$, training batch size $l$ \\
%\textbf{Output}: Sampling pattern $\Omega$
%\begin{algorithmic}[1]
%\State 
% \begin{tabular}{ccc} 
%\textbf{(SCG) }  Initialize $t=1$  
%    \end{tabular}
% \While{$c(\Omega) \leq \Gamma$}
%        
%        \State   $ \left \{\begin{tabular}{l}
% \textbf{(G) } Pick $\mathcal{S}_{iter} = \mathcal{S}$   \\
% \textbf{(SG) } Pick $\mathcal{S}_{iter}\subseteq \mathcal{S}$ at random, with $|\mathcal{S}_{iter}| = k$       \\
% \textbf{(SCG) } Pick $\mathcal{S}_{iter}\subseteq \mathcal{S}_t$ at random, with $|\mathcal{S}_{iter}| = k$  
%  \end{tabular} \right.$
%        \State   $ \left \{\begin{tabular}{l}
% \textbf{(v1) } Pick $\mathcal{L} = \{1,\ldots,m\}  $ \\
% \textbf{(v2) } Pick $\mathcal{L} \subseteq \{1,\ldots,m\} $, with $|\mathcal{L}| = l $
%  \end{tabular} \right.$
%         \For{$S \in \mathcal{S}_{iter} \text{ such that } |\Omega \cup S| \leq \Gamma$} 
%     
%        \State  $\Omega' = \Omega \cup S$ 
%        \State For each $\ell \in \mathcal{L}$ set $\*b_\ell\leftarrow \*P_{\Omega'}\bm\Psi\*x_\ell$, ${\hat{\*x}}_\ell\leftarrow g(\Omega',\*b_\ell)$
%        \State   $\eta(\Omega') \leftarrow \frac{1}{|\mathcal{L}|} \sum_{\ell\in\mathcal{L}} \eta(\*x_\ell, {\hat{\*x}}_\ell)$
% \EndFor
% \State $\displaystyle\Omega \leftarrow \Omega \cup S^*,  \text{ where }$   $\displaystyle S^* = \argmax_{\substack{S:|\Omega \cup S| \leq \Gamma}} \eta(\Omega\cup S) -\eta(\Omega)$
%\State   \textbf{ (SCG) }   $t= t \bmod T+1$  
%    \EndWhile
%\State {\bf return} $\Omega$ 
%\end{algorithmic}
%\end{algorithm} 

%\subsubsection{Stochastic greedy algorithms}
%To address the scalability issue of \textbf{G-v1}, we propose two complementary approaches. The first approach considers  a subset $\mathcal{S}_{iter}$ of $\mathcal{S}$, chosen either at random (Stochastic Greedy - \textbf{SG}), or at random \textit{from the $t$-th frame}, which will be denoted as $\mathcal{S}_{iter} \subseteq \mathcal{S}_{t}$ (Stochastic Cycling Greedy - \textbf{SCG}). Then, the same greedy procedure as Algorithm \ref{alg:1}.a is run, and at the end of an iteration, either a new subset of $\mathcal{S}$ is selected at random (Algo.~\ref{alg:1}.b), or the index of the selected frame is incremented (Algo.~\ref{alg:1}.c) and a subset is drawn at random from this frame. The number of samples used at each iteration is given by the batch size $k$. It is important to highlight that this approach preserves all the benefits of the previous greedy approach: our method remains nearly parameter free even when considering the batch size $k$. Empirical results in section \ref{sec:comp_greedy} suggest that the tuning of this parameter is simple and does not change the accuracy of  reconstruction when chosen as a reasonable fraction of the total number of phase encoding lines.
%
%The main difference between \textbf{SG} and \textbf{SCG} lies in the way the random subset is chosen. This difference has the practical implication that the sampling masks designed in Algorithm \ref{alg:1}.c will have the same number of samples per frame,  which is desirable for a dMRI scan \cite{ahmad2015variable}, as undersampling frames at different rates may alter the temporal resolution, thus leading to potentially missing critical temporal events. 
%
%
%The second approach, labelled as \textbf{v2} in Algorithm \ref{alg:1} increases the scalability of the algorithms by selecting at random a batch of training data of size $l$ for each iteration instead of cycling through the whole training set. Restricting ourselves to the case where full lines of $N$ sampling locations are added simultaneously to the mask, the complexities of the different flavours of these greedy algorithms are summarised below:
%
%\begin{table}[!t]
%\centering
%  \caption{Number of reconstructions performed by the different versions of Algorithm \ref{alg:1}. The result in bold denotes the speedup of Gv1 against SG-v2. $r$ denotes the target sampling rate, $n=rNT$.}\label{tab:nom}
%  \begin{tabular}{>{\bfseries}c | c c | c}
%    \toprule
%    &\textbf{G}& \textbf{SG} & \textbf{Speedup}\\
%    \midrule
%    v1 & $\Theta(mr(NT)^2)$ & $\Theta(mrkNT)$ & $ \Theta(NT/k)$\\
%    v2 & $\Theta(lr(NT)^2)$ & $\Theta(lrkNT)$& $\Theta(NT/k)$ \\ 
%     \midrule
%    \textbf{Speedup} & $\Theta(m/l)$ & $\Theta(m/l)$ & $\mathbf{\Theta(\frac{m}{l}\frac{NT}{k})}$\\ 
%    \bottomrule
%  \end{tabular}
%\end{table}
%
%
%
%
%%\subsubsection{Connexion to submodular optimization}
%%Additionally, in the field of submodular optimization, the stochastic greedy approach also has rigorous near-optimal guarantees \cite{mirzasoleiman2015lazier}.
%
%
%%The first one, \textbf{SG} and  \textbf{SCG}
%
%%Our main contribution is the scalable version of Algorithm \ref{alg:1}.a, which makes it suited to problems such as dMRI. 
%%To address the scalability issue of Algorithm \ref{alg:1}.a, we consider  a subset $\mathcal{S}_{iter}$ of $\mathcal{S}$, chosen either at random (Algo. \ref{alg:1}.b), or at random \textit{from the $t$-th frame}, which will be denoted as $\mathcal{S}_{iter} \subseteq \mathcal{S}_{t}$ (Algo. \ref{alg:1}.c). Then, the same greedy procedure as Algorithm \ref{alg:1}.a is run, and at the end of an iteration, either a new subset of $\mathcal{S}$ is selected at random (Algo.~\ref{alg:1}.b), or the index of the selected frame is incremented (Algo.~\ref{alg:1}.c) and a subset is drawn at random from this frame. The number of samples used at each iteration is given by the batch size $k$. It is important to highlight that this approach preserves all the benefits of the previous greedy approach: our method remains nearly parameter free even when considering the batch size $k$. Empirical results in section \ref{sec:comp_greedy} suggest that the tuning of this parameter is simple and does not change the accuracy of  reconstruction when chosen as a reasonable fraction of the total number of phase encoding lines. %Additionally, in the field of submodular optimization, the stochastic greedy approach also has rigorous near-optimal guarantees \cite{mirzasoleiman2015lazier}.
%
%
%%\subsection{Learning-based variable density}
%%An intuitive approach given in \cite{gozcu2017} is to find an approximative solution to the combinatorial problem \eqref{eq:erm}  by generating a set of candidate masks $\Omega_1,\dotsc,\Omega_{L}$ using parametric variable-density methods, and choose the one with the best empirical performance on the training set (Algorithm \ref{alg:4}). While similar ideas have already been used when performing parameter sweeps in existing works (e.g., see \cite{knoll2011adapted}), the framework of \cite{gozcu2017} justifies why the empirical performance is the correct quantity to optimize. 
%%\vspace{-.2cm}
%%\begin{algorithm}
%%
%%\caption{Learning-based variable density (LB-VD)}
%%\label{alg:4}
%%\textbf{Input}: Training data $\*x_1, \ldots, \*x_m$, reconstruction rule $g$, candidate masks $\Omega_1,\dotsc,\Omega_L$ \\
%%\textbf{Output}: Sampling pattern $\Omega$
%%\begin{algorithmic}[1]
%%\For{$\ell = 1,\dotsc,L$}
%%        \State For each $j$, set  $\*b_{j} \leftarrow \*P_{\Omega_{\ell}}\bm\Psi\*x_j$, $\hat{\*x}_j \leftarrow g(\Omega_{\ell},\*b_j)$ 
%%        \State $\eta_{\ell} \leftarrow \frac{1}{m}\sum_{j=1}^m \eta(\*x_j,\hat{\*x}_j)$
%% \EndFor
%% \State $\Omega \leftarrow \Omega_{\ell^*}$, where $\ell^* = \argmax_{\ell=1,\dotsc,L} \eta_{\ell}$
%% \State {\bf return} $\Omega$
%%\end{algorithmic}
%%\end{algorithm}
%
%
%


==> ICASSP_Scalable_MRI_arXiv copy/04-experiments.tex <==
%!TEX root = ms.tex
\vspace{-.5cm}
\section{Numerical Experiments}\label{sec:experiments}
\vspace{-.3cm}
\subsection{Implementation details}
\vspace{-.2cm}
%% % % % % % % % % % % % % % % % % % % % % % % % % %
%%% IMPLEMENTATION DETAILS
%% % % % % % % % % % % % % % % % % % % % % % % % % %
\textbf{Reconstruction algorithms:}  We consider three reconstruction algorithms, namely \textit{$k$-$t$ FOCUSS} (KTF) \cite{jung2009k},  and \textit{ALOHA} \cite{jin2016general}.  Their parameters were selected to maintain a good empirical performance across all sampling rates considered.

\textbf{Mask selection baselines:}\vspace{-.3cm}

\begin{itemize}[leftmargin=*]
%
\item\textit{Coherence-VD} \cite{lustig2007sparse}: We consider a random \textit{variable-density} sampling mask with Gaussian density and optimize its parameters to minimize coherence.
\item\textit{LB-VD} \cite{gozcu2017,gozcu2019rethinking}: Instead of minimizing the coherence as in \textit{Coherence-VD}, we perform a grid search on the parameters using the training set to optimize reconstruction according to the same performance metric as our method.
\end{itemize}
\textbf{Data sets:}  Our dynamic data were acquired in seven adult volunteers with a balanced steady-state free precession (bSSFP) pulse sequence on a whole-body Siemens 3T scanner using a 34-element matrix coil array. Several short-axis cine images were obtained during a breath-hold scan. Fully sampled Cartesian data were acquired using a $256\times 256$ grid with $25$ frames, then combined and cropped to  a $152 \times 152 \times 17$ single coil image. The details of the parameters used are provided in the supplementary material \cite{sanchez2018}. In the experiments, we used three volumes for training and four for testing. 

\vspace{-.4cm}
\subsection{Comparison of greedy algorithms}
\vspace{-.2cm}
We first compare the performance of \ga with SG-v1 and SG-v2, and show the results on Figure \ref{fig:psnr_batch}. We are specifically interested in determining the sensitivity of our algorithm to the sampling batch size $k$ and training batch size $l$ (for SG-v2, we use $l=1$ unless stated differently). We see that using a small batch size $k$ (e.g. $10$) yields a drop in performance, while $k=38$ even improves performance compared to G-v1, with respectively $60$ times less computation for \sga and $180$ less computations for SG-v2. One should also note that using a batch of training images (SG-v2) does not reduce the performance compared to SG-v1, while largely reducing computations. Also, additional results (in the supplementary material \cite{sanchez2018}) show that using larger batches yields similar results as for $k=38$. The fact that the performance of SG-v2 with $k=38$ outperforms G-v1 could be surprising, but originates in the lack of structure of the problem, where introducing noise in the computations  through random batches of samples improves the overall performance of the method. In the sequel, we use $k=38$ and $l=1$ for SCG-v2.

\begin{figure}[!tbp]

  \centering
  \begin{minipage}[b]{.58\linewidth}
 \hspace{-.3cm}\includegraphics[width=\linewidth]{main-figure0}
\end{minipage}\hfill
 \begin{minipage}[b]{.4\linewidth}
 \caption{PSNR as a function of the sampling rate for KTF, comparing the different reconstruction methods as well as the effect of the batch size on the quality of the reconstruction for SG. }\label{fig:psnr_batch}
 \end{minipage} 
  \vspace{-.8cm}
\end{figure}
\vspace{-.4cm}
\subsection{Single coil results}\label{sec:baseline_main} 
\vspace{-.2cm}
The comparison to baselines is shown on Figures \ref{fig:psnr_cross} and \ref{fig:plot_cross}, where we see that the SG-v2 method yields masks that consistently improve the results compared to all variable-density methods used. 


We notice in Figure \ref{fig:plot_cross} that comparing the reconstruction algorithms with VD methods do not allow for a faithful performance comparison of the reconstruction algorithms: the performance difference is very small between the reconstruction methods. In contrast, considering the reconstruction algorithm jointly with a sampling pattern optimized with our model-free approach makes the performance difference much more noticeable: ALOHA with its corresponding mask clearly outperforms KTF, and this conclusion could not be made by looking solely at reconstructions with VD-based masks. Note that extended results, along with multi-coil experiments, are available in our supplementary material \cite{sanchez2018}.

\begin{figure}[!t]
\centering
\vspace{-.7cm}
\hspace{-.3cm}\includegraphics[width=.95\linewidth]{main-figure1}
\vspace{-.5cm}
\caption{PSNR as a function of sampling rate for both reconstruction algorithms considered, comparing the mask design methods considered, averaged on $4$ images.}\label{fig:psnr_cross}
\vspace{-.5cm}
\end{figure}
%

\begin{figure}[!t]
\centering
\vspace{-.7cm}
\includegraphics[width=.95\linewidth]{main-figure2}
\vspace{-.4cm}
\caption{Comparison of the different reconstruction masks and decoders, for a sampling rate of $15\%$ on a single sample with its PSNR/SSIM performances.}\label{fig:plot_cross}
\vspace{-.5cm}
\end{figure}
\vspace{-.5cm}
\subsection{Large scale static results}
\vspace{-.3cm}

This last experiment shows the scalability of our method to very large datasets. We used the fastMRI dataset \cite{zbontar2018fastmri} consisting of knee volumes  and trained the mask for reconstructing the $13$ most central slices of size $320\times 320$, which yielded a training set containing $12649$ slices. For the sake of brevity, we only report computations performed using total variation (TV) minimization with NESTA \cite{becker2011nesta}. For mask design, we used the SG-v2 method with $k=80$ and $l=20$ (2500 fewer computations compared to G-v1). The LB-VD method was trained using $80$ representative slices and optimizing the parameters with a similar computational budget as SG-v2. The result on Figure \ref{fig:psnr_fastmri} shows a uniform improvement of our method over the LB-VD approach.

\begin{figure}[!t]
  \centering
 %  \vspace{-.5cm}
  \begin{minipage}[t]{.58\linewidth}
  \vspace{0pt}
 \hspace{-.3cm}\includegraphics[width=\linewidth]{main-figure3}
\end{minipage}\hfill
 \begin{minipage}[t]{.42\linewidth}
 \vspace{0pt}
 \caption{PSNR as a function of the sampling rate for TV, averaged on the 13 most central slices of the fastMRI validation set \cite{zbontar2018fastmri} (2587 slices). SGv2 outperforms LB-VD over all sampling rates.}\label{fig:psnr_fastmri}
  \vspace{-1cm}
 \end{minipage} 
   \vspace{-.8cm}
\end{figure}






==> ICASSP_Scalable_MRI_arXiv copy/05-conclusion.tex <==
%!TEX root = ms.tex
\vspace{-.3cm}
\section{Discussion and Conclusion}\label{sec:conclusion}
\vspace{-.3cm}
We presented a scalable sampling optimization method for dMRI, which largely addresses the scalability issues of  \cite{gozcu2017,gozcu2019rethinking}.  Reducing the resources used by \ga by as much as a $200$ times was shown to have no negative impact on the quality of reconstruction achieved within our framework. Our method was demonstrated to successfully scale to very large datasets such as fastMRI \cite{zbontar2018fastmri}, which the previous greedy method \cite{gozcu2017} could not achieve.

The masks obtained bring significant image quality improvements over the baselines. The results suggest that VD-based methods limit the performance of CS applied to MRI through their underlying model. They are consistently outperformed by our model-free and data-adaptive method on different \textit{in vivo} datasets, across several decoders, field of views and resolutions. Our findings highlight that sampling design should not be considered in isolation from data and reconstruction algorithm, as using a mask that is not specifically optimized can considerably hinder the performance of the algorithm.

More importantly, our theoretical results show that the generic non-convex Problem~\eqref{eq:emp} aiming at finding a probability mass  function under a cardinality constraint from which a mask is subsequently sampled, is equivalent to the discrete Problem~\eqref{eq:main emp equiv 2} of looking for the support of this PMF. This connection opens the door to rigorously leveraging techniques from combinatorial optimization for the problem of designing optimal, data-driven sampling masks for MRI.

%We also showed that our method largely resolves the scalability issues of \cite{gozcu2017,gozcu2019rethinking} by resorting to a stochastic greedy method, while preserving its advantages of being intuitive, versatile, and easy to pair with any reconstruction and anatomy.  Reducing the resources used in the greedy algorithm by as much as a $200$ times was shown to have no negative impact on the quality of reconstruction achieved within our framework. 

%Moreover, given a similar computational budget, they provide masks only for a few sampling rates and those masks are outperformed by our model-free greedy approach. % WE DON'T HAVE TO EMPHASIZE EVERY SINGLE ADVANTAGE IN THE CONCLUSION, THE MOST IMPORTANT ONES SHOULD BE HERE. 

 
%The significant present improvement over the state-of-the-art mask designs was achieved with a small number of training samples, and the application of our framework to larger scale datasets could further improve the quality of the optimized masks.  Moreover, we anticipate that the proposed framework could also greatly benefit other settings such as 3D (d)MRI and parallel imaging in general. 




%We presented an approach also brought significant improvements over state-of-the-art mask designs methods on two \textit{in vivo} datasets, consistently across several decoders, field of views and resolutions. \rev{We showed that the commonly used methods of parameter tuning and coherence minimization for variable-density approaches limit the performance of CS applied to MRI through their underlying model. Indeed, given a similar computational budget, they provide masks only for a few sampling rates and those masks are outperformed by our model-free greedy approach.
%
%    \rev{Additionally, our findings highlight that algorithmic design should not be considered in isolation from sampling design, as comparing algorithms on a same sampling pattern might not faithfully reflect its performance. } 
%    
% \rev{We showed that our method largely resolves the scalability issues of \cite{gozcu2017} by resorting to a stochastic greedy method,} while preserving its advantages of being intuitive, versatile, and easy to pair with any reconstruction and anatomy. Reducing the resources used in the greedy algorithm by as much as a $60$ times was shown to have no negative impact on the quality of reconstruction achieved within our framework.   
%    
% Our approach also brings a fixed mask obtained from a nearly parameter-free approach, whereas the VD approach relied on sampling from a tuned parametric distribution.} This solves an issue complicating the incorporation of compressed sensing-based methods into routine clinical MRI \cite{axel2016accelerated}. 
%
%The significant present improvement over the state-of-the-art mask designs was achieved with a very small number of training samples, and the application of our framework to larger scale datasets could further improve the quality of the optimized masks.  Moreover, we anticipate that the proposed framework could also greatly benefit applications like 3D (d)MRI and parallel imaging in general. 
